AEGIS: An Agent-based Framework for General Bug Reproduction from Issue Descriptions

In software maintenance, bug reproduction is essential for effective fault localization and repair. Manually writing reproduction scripts is a time-consuming task with high requirements for developers. Hence, automation of bug reproduction has increasingly attracted attention from researchers and practitioners. However, the existing studies on bug reproduction are generally limited to specific bug types such as program crashes, and hard to be applied to general bug reproduction. In this paper, considering the superior performance of agent-based methods in code intelligence tasks, we focus on designing an agent-based framework for the task. Directly employing agents would lead to limited bug reproduction performance, due to entangled subtasks, lengthy retrieved context, and unregulated actions. To mitigate the challenges, we propose an Automated gEneral buG reproductIon Scripts generation framework, named AEGIS, which is the first agent-based framework for the task. AEGIS mainly contains two modules: (1) A concise context construction module, which aims to guide the code agent in extracting structured information from issue descriptions, identifying issue-related code with detailed explanations, and integrating these elements to construct the concise context; (2) A FSM-based multi-feedback optimization module to further regulate the behavior of the code agent within the finite state machine (FSM), ensuring a controlled and efficient script generation process based on multi-dimensional feedback. Extensive experiments on the public benchmark dataset show that AEGIS outperforms the state-of-the-art baseline by 23.0% in F->P metric. In addition, the bug reproduction scripts generated by AEGIS can improve the relative resolved rate of Agentless by 12.5%.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> Sections/2_Empirical.tex <==
The quality of issue descriptions varies significantly~\cite{DBLP:journals/corr/abs-2407-01489}. Part of issue descriptions may directly include complete steps to reproduce the problems along with detailed code examples, while others may only provide general overviews to solve problems with natural language. These variations are related to the development experiences and writing styles of the issue raisers. Therefore, it is crucial to first assess the quality of issue descriptions and then figure out the difficulty of reproducing the coding problems in real-world development scenarios, which is essential to determine the necessity of designing more intelligent techniques to improve the performance of the bug reproduction task.

SWE-bench Lite~\cite{swebench} is a recently proposed benchmark that consists of issue descriptions and the corresponding open-source repositories, with the goal of automatically resolving the development problems presented in the issue (e.g., code fix, new feature update). In this dataset, any information that is temporally ahead of the issue submission time is not allowed to be used, which is highly consistent with the real-world software development process. As a most recent research, Agentless~\cite{DBLP:journals/corr/abs-2407-01489} has conducted an in-depth analysis of the dataset characteristics from several perspectives, including whether the issue description contains reproducible code examples, and the granularity of the code-fix locations involved in the issue content. For bug reproduction task, Agentless provides four levels to describe the extent of containing reproducible code examples in issue descriptions: (1) Contains Reproducible Example, (2) Contains Partial Reproducible Example, (3) Info in NL, and (4) Not Enough Info. After manually analyzing all cases, Agentless provides the proportions for each level: 54.7\%, 8.7\%, 27.3\%, and 9.3\%. It is notable that Agentless concludes that more than half of the cases in SWE-bench Lite dataset contain complete code examples for reproducing the problem, which seems rather high. Therefore, an obvious doubt arises from the analysis result: given the high quality of issue descriptions, with most cases seemingly requiring only the copying of relevant code snippets into the development environment for problem reproduction, is there still practical value in iterating more advanced approaches for this task?

To verify whether the situation is truly as Agentless claims, we conduct a reanalysis. Since SWE-bench Lite dataset consists of 12 open-source projects, for each of them, we randomly select 4 cases which are annotated as "Contains Reproducible Example" in Agentless. 
If a project contains fewer than 4 cases that meet the criteria, all available cases are selected. Based on this, we extract a total of 39 cases. We then design seven indicators from different perspectives to assess the completeness of the bug reproduction code embedded in the issue texts, which are as follows:

\textbf{(1) Input Example (IE).} This attribute is used to assess whether the issue description provides complete examples for the input objects. The forms of input objects are diverse. Sometimes they should be explicitly defined within the code. For example, in \textit{sympy-22005}, the reproduction code provided is 
\textit{solve\_poly\_system((x - 1,), x, y)}, but it does not specify the values for the identifiers \textit{x} and \textit{y}, making it an incomplete case that cannot be executed immediately. In another scenario such as \textit{pytest-11143}, only a reproduction command \textit{pytest -k xxx} is provided without any target test files to run, which also renders it incomplete. We have designed 3 options (i.e., \textit{complete}, \textit{partial}, and \textit{none}) to evaluate the extent of the input completeness in the issue description.

\textbf{(2) Import Dependency (ImD).} This attribute is leveraged to assess whether the issue description contains enough import information to ensure the normal execution of the provided reproduction code. 
%Evidently, incomplete import information also leads to additional workload, necessitating manual efforts to retrieve, verify, and adapt the relevant dependencies. 
For example, in \textit{seaborn-3010}, the identifier \textit{so} in the reproduction code \textit{so.Plot([1, 2, 3, None, 4], [1, 2, 3, 4, 5]).add(so.Line(), so.PolyFit())} is not pointed to a related import statement, making it an incomplete case. We have designed 5 options (i.e., \textit{complete\_code}, \textit{partial\_code}, \textit{natural language}, \textit{none}, and \textit{no\_need}) to evaluate the extent of the import completeness in the issue description. Note that, \textit{no\_need} indicates that the reproduction code can run without any import statements, which can also be considered as \textit{complete} in this particular scenario.

\textbf{(3) Run Configuration (RC).} This attribute is utilized to assess whether the issue description contains complete run configurations if needed. In many scenarios, the runtime environment needs to be pre-configured, or it is challenging to initiate the main reproduction code. For instance, in \textit{django-14017}, the reproduction code is \textit{Q(...) \& Exists(...)}, where the indispensable run configurations such as \textit{INSTALLED\_APPS} and \textit{DATABASES} within \textit{settings.configure} are not provided, resulting in a failed program execution. We leverage the same 5 options defined in (2) to evaluate the extent of the completeness of run configurations in the issue description.

\textbf{(4) Identifier Definition (IdenD).} This attribute is employed to assess whether all the used identifiers have explicit sources in the issue description. The undefined identifiers will cause runtime errors. Therefore, it is also an important attribute in assessing the quality of an issue description. For instance, in \textit{django-14915}, a statement in reproduction code is \textit{context = super().create\_option(name, ...)}, where the super class is not given, making the identifier \textit{create\_option()} unseen in this limited scope, which will cause runtime error. We have designed 2 options (i.e., \textit{none} and \textit{no\_need}) to evaluate the extent of the completeness of identifier definitions in the issue description, where \textit{none} indicates that at least one undefined identifier exists, while \textit{no\_need} indicates that no one exists.

\textbf{(5) Process Interaction (PI).} This attribute is designed to assess whether all process interaction behaviors are clearly specified in the issue description. In some scenarios, reproducing the problem requires process interactions, such as invoking command-line instructions to start a service and subsequently analyzing the results generated after the process terminates. 
%Since this procedure is generally more complex, it is more challenging to reproduce the problem when missing code examples and detailed descriptions in the issue content. 
For example, in \textit{sphinx-8720}, only a reproduction command is provided which is \textit{make html epub}, and the expected behavior is stated as \textit{module pages should not be created for epub by default}. Therefore, it appears necessary to initiate another process to aid in reproducing the problem (i.e., to create html pages and check if module pages exist). However, the implementation details are not mentioned in the issue description, making it more challenging to accomplish. We leverage the same 5 options defined in (2) to evaluate the extent of the completeness of process interaction descriptions in the issue description.

\textbf{(6) Actual Output (AO).} This attribute is used to assess whether the actual output behavior is explicitly given. The actual output is one important source for designing assert statements to reproduce the problem, as it helps determine whether the behavior of the updated code differs from the original erroneous behavior. Generally, it can be categorized into two types: one is to throw exceptions, such as \textit{InconsistentAxisTypesError...} in \textit{astropy-7746}, while the other is to output an unexpected result without exceptions, such as \textit{[(1,)]} in \textit{sympy-17022}. Regarding these two types, we have designed a total of 6 options (i.e., \textit{stack\_trace}, \textit{error\_message}, \textit{complete\_code}, \textit{partial\_code}, \textit{natural language}, \textit{none}) to evaluate the completeness of actual outputs in the issue description.

\textbf{(7) Expected Output (EO).} This attribute is leveraged to assess whether the expected output behavior is explicitly given. The expected output is another important source for designing assert statements, as it specifies the correct behavior that the updated code should achieve. Generally, it can also be categorized into two types: one refers to a scenario where exceptions are thrown before code update and no exceptions exist after code update. Since the descriptions related to "no exceptions exist" may be silence, we design an option called \textit{default} to represent this situation. The second type involves generating visible correct output after code update. We have designed 4 options (i.e., \textit{complete\_code}, \textit{partial\_code}, \textit{natural language}, and \textit{none}) for this type (5 in total)to evaluate the completeness of expected outputs in the issue description.

\input{Tables/empirical}

We consider an issue description to be truly complete only when all 7 indicators are explicitly stated. In such scenarios, a developer is expected to successfully reproduce the problem without any additional information. Specifically, we apply the following rule regarding the 7 indicators to judge whether the issue quality is good enough (i.e., with complete information) or not (i.e., with partial information):
\begin{equation}  \label{eq:empirical}
\resizebox{0.95\linewidth}{!}{
$ quality(i) = 
\left\{
\begin{array}{ll}  
  complete, & if\  IE(i)\ in \ \{"complete"\}\ \&\& \ ImD(i)\ in \ \{"c\_code", "no\_need"\}\ \&\& \\
  & RC(i)\ in \ \{"c\_code", "no\_need"\}\ \&\& \ IdenD(i)\ in \ \{"no\_need"\}\ \&\& \\
  & PI(i)\ in \ \{"c\_code", "no\_need"\}\ \&\& \\
  & (AO(i)\ in \ \{"s\_trace", "e\_msg", "c\_code"\}\ ||\ EO(i)\ in \ \{"c\_code", "default"\})\\
  partial, & else\\  
\end{array}  
\right\}
$
}
\end{equation}
where $i$ indicates the index of the 39 cases shown in Table~\ref{tab:empirical}, and abbreviations of tokens are also provided in the table header. After calculation, it is found that 14 cases contain complete information for code reproduction task, accounting for 35.9\%, while the remaining 25 cases only contain partial information, accounting for 64.1\%. If this proportion is extrapolated to all 164 cases which are considered \textit{Contains Reproducible Example} in Agentless~\cite{DBLP:journals/corr/abs-2407-01489}, the estimated number of cases which are considered truly complete in this paper would be 59. Under this stricter rule, the actual proportion of the truly-complete cases is 59/300 = 19.7\%. This analysis shows that the proportion of 54.7\% in Agentless~\cite{DBLP:journals/corr/abs-2407-01489} is an inflated figure. Based on the more detailed analysis including indicator selection, rule design, manual analysis and proportional estimation conducted in this paper, the actual proportion of truly-complete cases in SWE-bench Lite is approximately 19.7\% (59/300). This indicates that there is still significant room for developing intelligent techniques for bug reproduction tasks. Therefore, in this paper, we attempt to design an agent-based approach to further enchance the task performance.

==> Tables/RQ1.tex <==
\definecolor{darkgreen}{rgb}{0,0.5,0}
\newcommand{\cross}{\textcolor{red}{\textbf{\XSolidBrush}}}
\newcommand{\tick}{\textcolor{darkgreen}{\Checkmark}}

\begin{table}[!htbp]
    \caption{The comparison between existing benchmarks and IssueFixBench. PL, DCM, and PQC indicate programming languages, dataset construction method and pairing quality confirmation.}
    \footnotesize
    \centering
    \setlength{\tabcolsep}{0.4mm}
    % \begin{tabular}{p{1.8cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{2cm}|p{0.5cm}|p{1.6cm}|p{1.6cm}}
    \begin{tabular}{c|c|ccc|c|c|c|c}
    \toprule
    \textbf{Dataset} & \textbf{Format} &\textbf{\#Langs} & \textbf{\#Repos} & \textbf{\#Samples} & \textbf{DCM} & \textbf{PQC} & \textbf{Real-world} & \textbf{Tasks} 
\\
\midrule
MMLU 
& MCQ
& - 
& - 
& 15,908  
& AC
& \cross
& \tick
& code QA
\\

CodeQA
& QAP
& 2
& -
& 190,000
& GE
& \cross
& \cross
& code QA
\\

CS1QA
& QAP
& 1
& - 
& 9,237
& AC, MR
& \tick
& \tick
& code QA
\\

CodeApex
& MCQ
& -
& -
& 250
& MR
& \tick
& \tick
& code QA
\\

IssueFixBench-QA
& QAP
& 5
& 30
& 300
& AC, FF, MR
& \tick
& \tick
& code QA
\\ 
    \bottomrule
    \end{tabular}
    \label{tab:data_compare}
\end{table}

==> Tables/RQ_discuss.tex <==
% \begin{table}[tbp]
%     \caption{Influence of the Searcher Agent to \framework. The `Context' column indicates whether the method retrieves code from the codebase, while the `GoldFile' column specifies whether the method is provided with the bug file path.}
%     \footnotesize
%     \centering
%     \setlength{\tabcolsep}{0.2mm}
%     \begin{tabular}{clccccc}
%     \toprule
%        & \textbf{Method} & \textbf{Context} & \textbf{GoldFile} & $F \rightarrow P(\uparrow)$ & $F \rightarrow X(\uparrow)$ & $P \rightarrow P(\downarrow)$ \\ \midrule
%       \textbf{\multirow{6}{*}{LLM-Based}}& ZEROSHOT-AGENT(GPT35-turbo) & \tick &\cross & 6.0\% & 39.0\% & 33.0\% \\ 
%        & ZEROSHOT-AGENT(GPT4) & \tick &\cross & 7.7\% & 55.0\% & 42.0\% \\ 
%        & ZEROSHOT-AGENT(GPT4o) & \tick &\cross & 10.3\% & 54.3\% & 42.7\% \\ 
%       & ZEROSHOT-AGENT(GPT35-turbo) & \tick & \tick & 4.3\% & 48.3\% & 26.0\% \\ 
%        & ZEROSHOT-AGENT(GPT4) & \tick & \tick & 8.0\% & 56.3\% & 42.0\% \\ 
%        & ZEROSHOT-AGENT(GPT4o) & \tick & \tick & 9.7\% & 50.7\% & 46.3\% \\ 
%        \midrule
%         \textbf{\multirow{4}{*}{Agent-Based}} & AgentBaseline & \tick &\cross & 13.0\% & 48.0\% & 28.3\% \\ 
%         & AgentBaseline-bm25 & \tick &\cross & \% & \% & \% \\ 
%         & AgentBaseline & \tick &\tick & 16.0\% & 50.3\% & 26.3\% \\ 
%         & \textbf{\framework} & \tick &\cross & 36.0\% & 90.0\% & 9.0\% \\ 
%         & \textbf{\framework-bm25} & \tick & \cross & \% & \% & \% \\ 
%         & \textbf{\framework} & \tick & \tick & 36.3\% & 89.3\% & 10.7\% \\
        
%     \bottomrule
%     \end{tabular}
%     \label{tab:rq1}
% \end{table}


% \begin{table}[tbp]
%     \caption{Influence of the Searcher Agent to \framework. The `GoldFile' column specifies whether the method is provided with the bug file path.}
%     \footnotesize
%     \centering
%     \setlength{\tabcolsep}{0.2mm}
%     \begin{tabular}{clccccc}
%     \toprule
%        & \textbf{Method} & \textbf{GoldFile} & $F \rightarrow P(\uparrow)$ & $F \rightarrow X(\uparrow)$ & $P \rightarrow P(\downarrow)$ \\ \midrule
%       \textbf{\multirow{6}{*}{LLM-Based}}& ZEROSHOT-AGENT(GPT35-turbo) &\cross & 6.0\% & 39.0\% & 33.0\% \\ 
%        & ZEROSHOT-AGENT(GPT4) &\cross & 7.7\% & 55.0\% & 42.0\% \\ 
%        & ZEROSHOT-AGENT(GPT4o) &\cross & 10.3\% & 54.3\% & 42.7\% \\ 
%       & ZEROSHOT-AGENT(GPT35-turbo)& \tick & 4.3\% & 48.3\% & 26.0\% \\ 
%        & ZEROSHOT-AGENT(GPT4) & \tick & 8.0\% & 56.3\% & 42.0\% \\ 
%        & ZEROSHOT-AGENT(GPT4o) & \tick & 9.7\% & 50.7\% & 46.3\% \\ 
%        \midrule
%         \textbf{\multirow{3}{*}{Agent-Based}} & AgentBaseline &\cross & 13.0\% & 48.0\% & 28.3\% \\ 
%         & AgentBaseline-bm25 &\cross & \% & \% & \% \\ 
%         & AgentBaseline-goldfile&\tick & 16.0\% & 50.3\% & 26.3\% \\ \midrule
%         & \textbf{\framework}&\cross & 36.0\% & 90.0\% & 9.0\% \\ 
%         & \textbf{\framework-bm25} & \cross & \% & \% & \% \\ 
%         & \textbf{\framework-goldfile} & \tick & 36.3\% & 89.3\% & 10.7\% \\
        
%     \bottomrule
%     \end{tabular}
%     \label{tab:discuss}
% \end{table}


\begin{table}[tbp]
    \caption{Influence of the Searcher Agent to \framework.}
    \small
    \centering
    \setlength{\tabcolsep}{0.2mm}
    \begin{tabular}{lcccc}
    \toprule
       \textbf{Method} & $F \rightarrow P$ & \metricA & \metricB \\ \midrule
         AgentBaseline & 13.0 & 27.1 & 31.5 \\ 
         AgentBaseline-BM25 & 14.3 & 24.8 &  33.6 &  \\ 
         AgentBaseline-GoldFile& 16.0 & 31.8 & 37.8 \\ \midrule
         \textbf{\framework} 
& 36.0
& 40.0
& 80.0 \\ 
         \textbf{\framework-BM25}  
& 34.7
& 37.3
& 85.3 \\ 
         \textbf{\framework-GoldFile} 
& 36.3
& 40.6
& 77.2 \\
        
    \bottomrule
    \end{tabular}
    \label{tab:discuss}
\end{table}

==> Tables/empirical.tex <==
\definecolor{Moccasin}{RGB}{255, 228, 181}
\definecolor{lavender}{RGB}{230, 230, 250}
\definecolor{MistyRose}{RGB}{255, 228, 225}
\definecolor{Snow3}{RGB}{205, 201, 201}
\definecolor{DarkSeaGreen}{RGB}{200, 238, 200}
\definecolor{LightBlue2}{RGB}{178, 223, 238}
\definecolor{Khaki1}{RGB}{255, 246, 143}
\definecolor{SlateGray1}{RGB}{178, 206, 255}

\newcommand{\roundedbox}[2]{
  \tikz[baseline=(char.base)]\node[fill=#1, rounded corners=1mm, inner sep=1pt, text width=9mm, align=center] (char) {#2};
}

\newcommand{\pcode}{\roundedbox{Moccasin}{p\_code}}
\newcommand{\ccode}{\roundedbox{lavender}{c\_code}}
\newcommand{\nlang}{\roundedbox{MistyRose}{nl}}
\newcommand{\none}{\roundedbox{Snow3}{none}}
\newcommand{\noneed}{\roundedbox{DarkSeaGreen}{no\_need}}
\newcommand{\default}{\roundedbox{LightBlue2}{default}}
\newcommand{\emsg}{\roundedbox{Khaki1}{e\_msg}}
\newcommand{\strace}{\roundedbox{SlateGray1}{s\_trace}}
\newcommand{\partialcom}{\roundedbox{Moccasin}{partial}}
\newcommand{\complete}{\roundedbox{lavender}{complete}}

\begin{table}[tbp]
\caption{Case analysis for bug reproduction tasks. In the table header, \textit{Dep.} indicates \textit{Dependency}, \textit{Config.} indicates \textit{Configuration}. In the table body, \textit{c\_code} indicates \textit{complete\_code}, \textit{p\_code} indicates \textit{partial\_code}, \textit{e\_msg} indicates \textit{error\_message}, \textit{s\_trace} indicates \textit{stack\_trace}, \textit{nl} indicates \textit{natural language}.}
\scriptsize
\label{tab:empirical}
\centering
\begin{tabular}{l|ccccc|cc|c}
\toprule
\textbf{Case ID} & \textbf{\begin{tabular}[c]{@{}c@{}}Input\\ Example\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Import\\ Dep.\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Run\\ Config.\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Identifier\\ Definition\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Process\\ Interaction\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Actual\\ Output\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Expected\\ Output\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Issue\\ Quality\end{tabular}}\\
\midrule
% \multicolumn{1}{c}{\textbf{Case ID}} & \multicolumn{1}{c}{\textbf{Trigger Condition}} & \multicolumn{1}{c}{\textbf{Actual Output}} & \multicolumn{1}{c}{\textbf{Expected Output}} & \multicolumn{1}{c}{\textbf{Import Dependency}} & \multicolumn{1}{c}{\textbf{Run Config.}} & \multicolumn{1}{c}{\textbf{Identifier Definition}} & \multicolumn{1}{c}{\textbf{Process Interaction}} & \multicolumn{1}{c}{\textbf{Input Example}} \\
1. django-14017 & \complete & \none & \none & \none & \noneed & \strace & \default & \partialcom \\

2. django-11422 & \complete & \noneed & \none & \noneed & \nlang & \nlang & \nlang & \partialcom \\

3. sympy-14774 & \none & \none & \noneed & \noneed & \noneed & \ccode & \ccode & \partialcom \\

4. django-14915 & \partialcom & \none & \none & \none & \noneed & \emsg & \default & \partialcom \\

5. sympy-22005 & \none & \none & \noneed & \noneed & \noneed & \ccode & \nlang & \partialcom \\

6. sympy-17022 & \complete & \pcode & \none & \noneed & \noneed & \ccode & \ccode & \partialcom \\

7. sympy-21171 & \complete & \ccode & \noneed & \noneed & \noneed & \strace & \default & \complete \\

8. matplotlib-23987 & \complete & \ccode & \noneed & \noneed & \noneed & \emsg & \default & \complete \\

9. scikit-learn-13142 & \complete & \ccode & \noneed & \noneed & \noneed & \strace & \default & \complete \\

10. matplotlib-23964 & \complete & \ccode & \noneed & \noneed & \noneed & \strace & \nlang & \complete \\

11. django-16041 & \complete & \pcode & \none & \noneed & \noneed & \nlang & \default & \partialcom \\

12. scikit-learn-13584 & \complete & \ccode & \noneed & \noneed & \noneed & \emsg & \default & \complete \\

13. pytest-11143 & \none & \none & \noneed & \noneed & \nlang & \strace & \default & \partialcom \\

14. pytest-7373 & \complete & \ccode & \noneed & \noneed & \nlang & \nlang & \nlang & \partialcom \\

15. seaborn-3010 & \complete & \none & \noneed & \noneed & \noneed & \strace & \default & \partialcom \\

16. matplotlib-25442 & \complete & \ccode & \noneed & \noneed & \noneed & \strace & \default & \complete \\

17. matplotlib-23562 & \complete & \ccode & \noneed & \noneed & \noneed & \strace & \default & \complete \\

18. pylint-5859 & \complete & \noneed & \noneed & \noneed & \nlang & \ccode & \ccode & \partialcom \\

19. scikit-learn-13241 & \none & \none & \noneed & \noneed & \noneed & \ccode & \nlang & \partialcom \\

20. scikit-learn-10297 & \complete & \ccode & \noneed & \noneed & \noneed & \emsg & \nlang & \complete \\

21. astropy-14995 & \complete & \ccode & \noneed & \noneed & \noneed & \emsg & \default & \complete \\

22. xarray-5131 & \complete & \ccode & \noneed & \noneed & \noneed & \ccode & \nlang & \complete \\

23. pytest-5413 & \complete & \none & \noneed & \noneed & \noneed & \nlang & \pcode & \partialcom \\

24. sphinx-8721 & \none & \noneed & \none & \noneed & \none & \nlang & \nlang & \partialcom \\

25. astropy-12907 & \complete & \ccode & \noneed & \noneed & \noneed & \ccode & \nlang & \complete \\

26. sphinx-8282 & \partialcom & \noneed & \pcode & \noneed & \nlang & \nlang & \nlang & \partialcom \\

27. seaborn-2848 & \complete & \none & \noneed & \noneed & \noneed & \emsg & \default & \partialcom \\

28. requests-2317 & \none & \noneed & \none & \noneed & \noneed & \nlang & \nlang & \partialcom \\

29. astropy-14182 & \complete & \ccode & \noneed & \noneed & \noneed & \strace & \default & \complete \\

30. pylint-7114 & \partialcom & \noneed & \noneed & \noneed & \ccode & \emsg & \default & \partialcom \\

31. sphinx-8595 & \partialcom & \noneed & \pcode & \noneed & \nlang & \nlang & \nlang & \partialcom \\

32. pytest-5103 & \complete & \noneed & \noneed & \none & \noneed & \ccode & \ccode & \partialcom \\

33. pylint-7080 & \none & \noneed & \ccode & \noneed & \nlang & \ccode & \nlang & \partialcom \\

34. pylint-7993 & \none & \noneed & \ccode & \noneed & \nlang & \ccode & \ccode & \partialcom \\

35. sphinx-7738 & \partialcom & \noneed & \nlang & \noneed & \nlang & \nlang & \nlang & \partialcom \\

36. seaborn-3190 & \complete & \none & \noneed & \noneed & \noneed & \strace & \default & \partialcom \\

37. xarray-4094 & \complete & \none & \noneed & \noneed & \noneed & \emsg & \default & \partialcom \\

38. astropy-7746 & \complete & \ccode & \noneed & \noneed & \noneed & \strace & \default & \complete \\

39. seaborn-3407 & \complete & \ccode & \noneed & \noneed & \noneed & \strace & \default & \complete \\
\bottomrule
\end{tabular}
\end{table}
